Hadoop in Low-Power Processors

In our previous work we introduced a so-called Amdahl blade microserver that combines a low-power Atom processor, with a GPU and an SSD to provide a balanced and energy-efficient system. Our preliminary results suggested that the sequential I/O of Amdahl blades can be ten times higher than that a cluster of conventional servers with comparable power consumption. In this paper we investigate the performance and energy efficiency of Amdahl blades running Hadoop. Our results show that Amdahl blades are 7.7 times and 3.4 times as energy-efficient as the Open Cloud Consortium cluster for a data-intensive and a compute-intensive application, respectively. The Hadoop Distributed Filesystem has relatively poor performance on Amdahl blades because both disk and network I/O are CPU-heavy operations on Atom processors. We demonstrate three effective techniques to reduce CPU consumption and improve performance. However, even with these improvements, the Atom processor is still the system's bottleneck. We revisit Amdahl's law, and estimate that Amdahl blades need four Atom cores to be well balanced for Hadoop tasks.

==> ack.tex <==
\section{Acknowledgments}
\label{sec:ack}
We would like to thank Rich Ercolani for help us manage the Amdahl cluster
and provide support for our work. We thank the people from
University of Chicago, Robert Grossman and Michal Sabala, for providing us
the Open Cloud Consortium cluster.

==> mapreduce.tex <==
\section{Map-Reduce Paradigm}
\label{sec:mapreduce}

There are two phases in the Map-Reduce programming paradigm. Mappers read data
from different input source, format it into records and pass them to a map
function. In the Hadoop framework, programmers can customize the 
form of an input record by extending some Java classes. The map function is one
of the major places where programmers put their programming logic. What a
programmer usually does is to assign keys to the record from the input 
data. In each map invocation, only one record is processed, so the map task is
very independent, which is good for massive parallel processing.

After the mapping phase, data is shuffled to reducers. When a reducer gets all
data it needs, it sorts the data so that the records with the same key are
gathered and one reduce invocation can process all values associated to the 
same key. The reduce function is the other place where programmers can insert
their logic.

In this model, when data is output by mappers, it is partitioned and the number
of partitions is defined by the number of reducers, i.e., each reducer gets a
partition from each mapper. There are some optimizations in this part to 
reduce the number of disk IO. Since Hadoop v0.17, it works as follow: when data
is output from a mapper, it is buffered in the memory whose maximal size is
configured in advance. There are two buffers for this purpose. One buffer is 
used to store the output data from mappers and the other is to store the
metadata for the output data. Whenever the size of the data (either in the data
buffer or the metadata buffer) reaches a threshold, it is sorted and spilled to
the 
disk. After a mapper outputs all data, it reads spilled data and does another
merge sorting and writes data back to the disk. If the buffer in the memory is
large enough, i.e., the size of output data never reaches the threshold, 
one disk writing and disk reading can be saved.

The execution of mappers and reducers can be overlapped, but the reducers can
start to sort the data and process it only after all mappers finish running.
While mappers are running, reducers can only pull data from the mappers.

In many cases, data is read from and written to a distributed file system. It is
Hadoop Filesystem (HDFS) in the Hadoop framework, which is implemented in the
user space. Thus, the performance of HDFS is vital to the performance of 
the whole system, especially when the user's own logic does not consume much CPU
time. A large file in HDFS is split into many blocks and the default size of a
block is 64MB. By default, a block of data is assigned to a mapper and 
the block of data is called a split. The number of splits decides the number of
mappers.

